Learning Safe Policies with Expert Guidance

We propose a framework for ensuring safe behavior of a reinforcement learning agent when the reward function may be difficult to specify. In order to do this, we rely on the existence of demonstrations from expert policies, and we provide a theoretical framework for the agent to optimize in the space of rewards consistent with its existing knowledge. We propose two methods to solve the resulting optimization: an exact ellipsoid-based method and a method in the spirit of the "follow-the-perturbed-leader" algorithm. Our experiments demonstrate the behavior of our algorithm in both discrete and continuous problems. The trained agent safely avoids states with potential negative effects while imitating the behavior of the expert in the other states.

==> algorithm.tex <==
\section{Algorithm}\label{sec:alg.}
\subsection{Follow the perturbed leader}
The agent is in an MDP without a specified reward function. Instead, the agent is presented with expert policy and features $\pi_E$ and $\mu_E$. The mapping between the policy and features $\phi$ is also known. This expert policy could be acquired by human demonstration or learned from an MDP that has all properties of the current MDP and a known reward function. We assume that we have access to an RL algorithm that can learn the optimal policy given a full MDP, so that we have the expert policy and thus the features. Recall the max-min goal as in equation \ref{def:max-min}, we will learn a roughly max-min solution using FPL. Our algorithm to learn such a policy $\tilde \pi$ is as follows:
\todo{Say adaptive adversary.}

Upon termination, the algorithm returns ${\tilde{\mu}} = 1/T \sum_{i=1}^T \mu_i $ and the corresponding ${\tilde {\pi}} $


==> model_based_exact_solver.tex <==
\section{Model-Based Learning using an Exact MDP Solver}~\label{sec:model based}
\subsection{Exact max-min solution with dual methods for MDPs}

Given a policy $\pi$, we can calculate the occupancy measure $x^\pi$ for all state and action pair as
\begin{equation}
	x^\pi_{sa} = E [\sum_{t=0}^\infty \gamma^t \mathbbm{1}_{s_t = s, a_t = a} | \pi , P_{sa}].
\end{equation}
This measures the expected and discounted number of visits to each state-action pair following the policy $\pi$. It requires the knowledge of the transition probabilities. The expectation has also taken into account the initial state distribution.The policy's expected reward can be represented as a linear function over the occupancy measure 
\begin{equation}
	V(\pi) := \sum_{s, a}R_{sa} x^\pi_{s a}.
\end{equation}
Similarly, we can express $\mu(\pi)$ as:
\begin{equation}
	\Psi(\pi) := \sum_{s} \phi(s) \sum_{a} x^\pi_{s a}
\end{equation}
Thus, we can replace the constraints on $\mu$ in our max-min problem with the {\it Bellman flow constraints} \cite{Puterman14}, and rewrite the max-min LP as following.

\begin{align*}
 &\max z &\\
 &z \leq \mu \cdot w,  \qquad \forall w \in P_R &\\
&\mu = \sum_{s} \phi(s) \sum_{a} x_{s a} &\\
& \sum_a x_{sa} = \Pr(s_0 = s) + \gamma \sum_{s',a}x_{s'a} P_{sa} \qquad \forall s &\\
& x_{sa} \geq 0 &\\
\end{align*}


==> related.tex <==
\section{Related Work}\label{sec:related}

In the sense of using expert demonstrations, our work is related to inverse reinforcement learning and apprenticeship learning~\cite{NgR00,AbbeelN04,SyedS08,SyedBS08}. In particular, the apprenticeship learning problem was formulated as a maxmin problem in~\cite{SyedS08,SyedBS08}. Despite the seemingly similarity, our maxmin learning problem aims to solve a completely different problem than apprenticeship learning. Here is a simple example: the expert is consistent with two reward functions $w_1$ and $w_2$ with $\epsilon = 25$. Say the expert gets 100 under $w_1$ and 70 under $w_2$, and the only alternative policy gives 90 and 90. Apprenticeship learning will return the expert policy while ours will return the latter solution. In the worst case (under $w_2$), our maxmin policy has better guarantees and thus is more robust.
We do not infer a specific reward function or imitate expert trajectories directly, but rather use them to provide information about the potential reward function. %(see \cite{HusseinGEJ17} for a survey).

\notshow{\paragraph{Apprenticeship Learning} Similarity: maxmin formulation, expert guidance. Difference: apprenticeship hopes to imitate the expert's behavior. We just want to infer consistent rewards from the expert and then do maxmin planning. Give example. Different application: we can accommodate multiple experts and do not need the training domain to be the same as testing domain. See experiment.~\cite{SyedBS08,SyedS08}}

Inverse reward design~\cite{HadfieldMARD17}  uses a proxy reward and infers the true reward by estimating its posterior. Then it uses risk-averse planning together with samples from the posterior in the testing environment to achieve safe exploration. Our approach achieves a similar goal without assuming any distribution over the rewards and is arguably more robust. We apply a single reward function to the whole MDP while they apply (maybe too pessimistically) per step/trajectory maxmin planning. Furthermore, our algorithm is guaranteed to find the maxmin solution in poly time, and it naturally accommodates multiple experts. 

Robust Markov Decision Processes  \cite{NilimEG05,Iyengar05}  have addressed the problem of performing dynamic programming-style optimization environments in which the transition probability matrix is uncertain. Lim, Xu \& Mannor \cite{LimXM13} have extended this idea to reinforcement learning methods.  This body of work also uses min-max optimization, but because the optimization is with respect to worst-case transitions, this line of work results in very pessimistic policies.  Our algorithmic approach and flavor of results are also different.
\cite{MorimotoD05} have addressed a similar adversarial setup, but in which the environment designs a worst-case disturbance to the dynamics of the agent, and have addressed this setup using $H_\infty$ control. 

%Our approach is also related in spirit to work in inverse reinforcement learning \cite{NgR00}, in which a reward function is inferred from expert demonstrations, and then optimized by the agent.  However, we do not infer a specific reward function, but rather use the incomplete expert data as prior knowledge for the optimization.  The relationship of our work to imitation learning%~\cite{AbbeelN04, AbbeelCQN07} 
%is similar - we do not imitate expert trajectories directly, but rather use them to provide information about the potential reward function (see \cite{HusseinGEJ17} for a survey).

